Reward Advancement: Transforming Policy under Maximum Causal Entropy Principle

Many real-world human behaviors can be characterized as a sequential decision making processes, such as urban travelers choices of transport modes and routes (Wu et al. 2017). Differing from choices controlled by machines, which in general follows perfect rationality to adopt the policy with the highest reward, studies have revealed that human agents make sub-optimal decisions under bounded rationality (Tao, Rohde, and Corcoran 2014). Such behaviors can be modeled using maximum causal entropy (MCE) principle (Ziebart 2010). In this paper, we define and investigate a general reward trans-formation problem (namely, reward advancement): Recovering the range of additional reward functions that transform the agent's policy from original policy to a predefined target policy under MCE principle. We show that given an MDP and a target policy, there are infinite many additional reward functions that can achieve the desired policy transformation. Moreover, we propose an algorithm to further extract the additional rewards with minimum "cost" to implement the policy transformation.

==> 02_preliminary.tex <==
%\section{Preliminaries and Problem Definition}
\section{Preliminaries}
\label{sec:pre}
  
%preliminaries.tex

%In this section, we briefly review the basics of finite Markov Decision Process and Maximum Entropy Inverse Reinforcement Learning, which are  the foundations of our data-driven model and inverse learning algorithm for urban passenger preferences characterization.

In this section, we review the basics of finite Markov Decision Process and Maximum Causal Entropy (MCE) policy. 
%We will define the reward advancement problem and outline our proposed solution framework.

\subsection{Markov Decision Process (MDP)}
%
An MDP is represented as a tuple $\langle S, A, T, \gamma, \mu_0, R\rangle$,
where $S$ is a finite set of states and $A$ is a set of actions. 
%
$T$ is the probabilistic transition function with $T(s'\mid s,a)$
as the probability of arriving at state $s'$ by executing
action $a$ at state $s$, $\gamma \in (0,1]$ is the discounting factor\footnote{Without loss of generality, we assume $\gamma=1$ in this paper, where our results can be extended to the case with $\gamma \in (0,1]$.},
$\mu_0: S\rightarrow [0,1]$ is the initial distribution, and
$R:S\times A\rightarrow \reals$ is the reward function. 
%In our problem, the \ac{mdp} has a set of terminal, sink states $S_\terminal$. It is ensured that every trajectory ends in one of the terminal states.
%  We assume that
% the reward function $r$ is given by a linear combination of feature
% vectors $\phi(s,a)$ with weights $\theta$ such that
% $r(s,a)\simeq \theta^T \phi(s,a)$ for $(s,a) \in S\times A$.
A randomized, memory-less policy is a function that specifies a probability distribution on the action to be executed in each state, defined as $\pi: S \times A\rightarrow [0,1]$.
%
The planning problem in an MDP aims to find a policy $\pi$, such that the
expected total reward is maximized, namely, 
\begin{align}
\pi^\ast &= \arg\max_{\pi\in \Pi}\mathbb{E}^\pi(\sum_{t=0}^T \gamma^t
R(S_t,A_t) \mid S_0\sim \mu_0), \label{eq:opt_pi}
\end{align}
where $S_t$ and $A_t$ are random variables for the state and action at
the time step $t$, and $T\in \reals\cup\{\infty\}$ is the set of time horizons. 
%
The initial state
$S_0$ follows the initial distribution $\mu_0$. Here, $\Pi$ is the
memory-less policy space.

\subsection{Policy under Maximum Causal Entropy Principle}

Optimal policy outlined in eq.(\ref{eq:opt_pi}) achieves the highest expected reward for the agent. It is widely used for machine (i.e., robot) agent design~\cite{ng2000algorithms,levine2014learning,li2004iterative}, where {\em perfect rationality} can be safely assumed~\cite{li2004iterative}. 
%
However, many studies have revealed that decisions made by human agents (even experts) are probabilistic and sub-optimal~\cite{kuefler2017imitating,wu2017data,tao2014examining}. These phenomena indicate that {\em human agents} are making decisions with bounded rationality~\cite{wu2017data,tao2014examining}, where actions are chosen with probabilities corresponding to the expected future rewards they are leading to. %
As a result, various inverse reinforcement learning algorithms were proposed to recover the reward function, $R: S\times A\rightarrow \mathbb{R}$ such that the distribution of action and state sequence under a near-optimal policy match the demonstrated human behaviors. 

One well-known solution to the inverse reinforcement learning problem is Maximum Causal Entropy Inverse Reinforcement Learning~\cite{ziebart2010modeling}. It proposes to find the policy that best represents demonstrated behaviors with highest causal entropy, which is summarized as follows.

\noindent{\bf Conditional Entropy}
 is used to measure the uncertainty of one distribution $A$ based on a given side information $S$, i.e., $H({A}|{S})=-\sum_{a\in A}\sum_{s\in S}P(s,a)\ln P(a|s)$. 

\noindent{\bf Causal Entropy} measures the uncertainty present in the causally conditioned
distribution of a sequence variable $A_{0:T}$, given the preceding partial sequences $S_{0:t}$ and $A_{0:t-1}$, with $0\leq t\leq T$. It
can be interpreted as the expected number of bits needed to encode the sequence $A_{0:t}$ given the
previous $A_{0:t-1}$ variables and sequentially revealed side information, $S_{0:t}$, which has been revealed at
each point in time and excluding unrevealed future side information, $S_{t+1:T}$, which is $H(A||S)=\sum_{t=0}^{T}H(A_t|A_{0:t-1},S_{0:t}).$

When the sequence is Markovian, we have $P(A_t|A_{0:t-1},S_{0:t})=P(A_t|S_{t}).$
Then, the causal entropy can be written as
$H(A||S)=\sum_{t=0}^{T}H(A_t|S_{t})$. As a result, the causal entropy of an MDP is characterized as eq.(\ref{eq:CE}) with $A$ and $S$ as the action sequence and the state sequence (side information), respectively.

\begin{align}
    H(A||S)&=\sum_{0\leq t\leq T}H(A_t|S_t)\\
    &=-\sum_{0\leq t\leq T}\sum_{s_t\in S}\sum_{a_t\in A}P(s_t,a_t)\ln \pi(a|s) \\
    &=-\sum_{s\in S}\sum_{a\in A}D(s,a)\ln\pi(a|s), \label{eq:CE}
\end{align}
where $P(s_t,a_t)$ is the joint probability of visiting a particular state-action pair $(s_t,a_t)$ at step $t$. $D(s,a)$ represents the expected visitation frequency of the state-action pair $(s,a)$, when one trajectory is generated under policy $\pi(a|s)$.

The policy under maximum causal entropy principle (i.e., {\em MCE policy}) best represents the demonstrated behaviors with the highest causal entropy, and is subject to the constraint of matching reward expectations to the distribution of demonstrated behaviors. Denote $Q(s,a)=R(s,a)+\sum_{s^\prime\in S}T(s^\prime|s,a)\sum_{a^\prime\in A}\pi(a^\prime|s^\prime)Q(s^\prime,a^\prime)$ as Q-function on state-action pair $(s,a)$, indicating the expected rewards to be received starting from $(s,a)$, MCE policy can be formulated as the following maximum causal entropy problem: 

\begin{align}
\textbf{Problem 1:} &\textbf{ Maximum Causal Entropy Policy:}\nonumber \\
\max_{\pi(a|s)}\quad\quad & H(A||S)=-\sum_{s\in S}\sum_{a\in A}D(s,a)\ln\pi(a|s),\label{eq:MCE_obj} \\ 
%-\sum_{s\in S}\sum_{a\in A}D(s,a)\log\pi(s,a),\\
s.t. \quad\quad&\sum_{s\in S}\sum_{a\in A}\mu_0(s)\pi(a|s)Q(s,a)=\tilde{Q}, \label{eq:MCE_c1} \\
&\sum_{a\in A}\pi(a|s)=1,\forall s\in S.\label{eq:MCE_c2}
\end{align}
where $\tilde{Q}=\sum_{\zeta\in\tilde{TR}}R(\zeta)/|\tilde{TR}|$ is expected empirical rewards which can be extracted from the behavior data. $\tilde{TR}=\{\zeta\}$ is a set of demonstrated trajectories from a human agent, and $|\tilde{TR}|$ denotes the size of the trajectory set. $R(\zeta)=\sum_{(s,a)\in \zeta}R(s,a)$ is the reward received on trajectory $\zeta$.

%and $\sum_{s\in S,a\in A}D(s,a)\log\pi(s,a)$ is the causal entropy. 


\begin{theoremm}\label{thm:theorem_Q_softmax}
The MCE policy characterized in {Problem 1} eq.(\ref{eq:MCE_obj})--(\ref{eq:MCE_c2}) follows the softmax format, 
$\pi(a|s)=\frac{e^{Q(s,a)}}{\sum_{a^\prime \in A}e^{Q(s,a^\prime)}}$.
\end{theoremm}
\begin{proof}	
This can be proven by introducing Lagrangian multipliers for constraints, and letting the derivative of Lagrangian function be zero. See more details in the supplementary material.
\end{proof}

%Eq.(\ref{eq:Qpi}) is the policy conducted by the human agent, that best matches her generated trajectory data.
%
%Usually, the $Q(s,a)$ can be represented using a parameterized function $Q(s,a|\theta)$, for instance, a neural network model. 
%
%The Q-function $Q(s,a|\theta)$'s can be estimated by solving a maximum likelihood estimation problem (See details in the supplementary material),
%\begin{align}
%\theta^* = \argmax \theta L(\theta) = \argmax \theta  \sum_{\zeta\in\tilde{TR}}\ln P(\zeta|\theta).
%\end{align}


%with ζ∈TR gradient decent method [2].



